Towards Interactive, Adaptive and Result-aware Big Data Analytics

As data volumes grow across applications, analytics of large amounts of data is becoming increasingly important. Big data processing frameworks such as Apache Hadoop, Apache AsterixDB, and Apache Spark have been built to meet this demand. A common objective pursued by these traditional cluster-based big data processing frameworks is high performance, which often means low end-to-end execution time or latency. The widespread adoption of data analytics has led to a call to improve the traditional ways of big data processing. There have been demands for making the analytics process more interactive and adaptive, especially for long running jobs. The importance of initial results in the iterative process of data wrangling has motivated a result-aware approach to big data analytics. This dissertation is motivated by these calls for improvement in data processing and the experiences over the past few years while working on the Texera project, which is a collaborative data analytics service being developed at UC Irvine. This dissertation mainly consists of three parts. The first part is about the design of the Amber engine that serves as the backend data processing framework for the Texera service. The second part is about an adaptive and result-aware skew-handling framework called Reshape. Reshape uses fast control messages to implement iterative skew mitigation techniques for a wide variety of operators. The mitigation techniques in Reshape have also been analyzed from the perspective of their effects on the results shown to the user. The last part is about a result-aware workflow scheduling framework called Maestro. This part talks about how to schedule a workflow for execution on computing clusters and make result-aware decisions while doing so. This work improves the data analytics process by bringing interactivity, adaptivity and result-awareness into the process.

==> chap2-amber/sec5.tex <==

\section{Real-time Processing of Control Messages}
\label{sec:realtime-controlmessage-processing}

%During the execution of a workflow, if the user has some inkling about erroneous results and wants to enter the debug mode, the engine should support real-time interaction and debugging, and quick processing of control messages is critical. 

A critical requirement in the Spartan system is fast processing of control messages in order to support real-time interaction and debugging.  In this section, we first study how to make a control message available to an actor quickly, then discuss how an actor behaves after receiving a {\sf Pause} message and a {\sf Resume} message, respectively.

\subsection{Expedited Processing of Control Messages}

Worker actors process a large number of data messages in addition to control messages. These two types of messages to a worker actor are enqueued in the same mailbox, which is a FIFO queue in the actor model. Therefore, there is a delay between the enqueuing of a control message and its processing, which is affected mainly by two factors. {\em 1. Number of enqueued messages.} The worker actor has to process all the messages already present in the mailbox, before it can process a newly enqueued message. For a large amount of data, workers can have many data batches queued in their mailbox. {\em 2. Computation per batch.} Even if there is only one data message ahead of a control message in the mailbox, the data message can take a long time to process. For example, some machine learning (ML) operators can take seconds to process a single tuple.  The needs for user interaction necessitates quick processing of control messages once they arrive in the mailbox. An obvious solution is to give a higher priority to control messages, so that they can be processed before data messages. Some actor model implementations such as Akka do allow priority-based mailboxes, but the actor model specification natively does not provide such support, and we want the Spartan engine to be general without depending on a specific actor model implementation.

% Taking the two factors into consideration, suppose there are $n$ data messages before a control message in the mailbox, each data message contains a batch of $\alpha$ tuples, and each tuple takes time $\beta$ to process, then the delay between the arrival of the control message and the start of its processing is:

% \begin{equation}
%     delay \approx n \alpha  \beta.
% \end{equation}

% Assuming a FIFO-based mailbox, where there are $n$ data messages before a control message

We will use a {\sf Pause} request as an example to discuss expedited control message processing, and the idea can be generalized to other control messages as well.  Consider the following two solutions.

\vspace{0.05in}
\noindent \textbf{Solution 1. Delayed processing of data messages.} For each data batch, the worker processes a few tuples (say $\tau$) and saves the remaining tuples in the batch in its internal state. Then the worker sends itself a {\sf Process-Saved-Batch} control message to remind itself to process the saved batches. The purpose is to reduce the time to process this batch, and provide an opportunity to a control message in the mailbox to be processed.  When the actor receives the {\sf Process-Saved-Batch} message sent by itself, it again processes $\tau$ tuples and resends the same message to itself. As $\tau$ decreases, the delay decreases, but the number of messages in the system increases, which could clog the network and affect the flow of control messages between actors. If $\tau$ is too small, the results can be antithetical to the aim of real-time debugging and interaction.  


% The approach is illustrated in the code snippet below.

% \begin{algorithm}[ht]
%   \SetKwFunction{ProcessBatch}{Process-Batch}
%   \SetKwProg{myproc}{Procedure}{}{}
%   \myproc{\ProcessBatch{}}{
%     \For{$i \gets 1$ \textbf{to} $\tau$} {
%         Process $batch[i]$\;
%     }
%     Save batch[$\tau$+1 \ldots batch.size()] in the actor's internal state\;
%     Send a {\sf Process-Saved-Batch} message to itself\;
%     }{}
%   \caption{Solution 1}
% \end{algorithm}

% \begin{algorithmic}
% \Procedure{Process-Batch}{$batch$}
 %   \For{$ i \in \{1\ldots\tau \} $}
%     \State Process batch[i]
%   \EndFor
%   \State Save batch[$\tau$+1 \ldots batch.size()] in actor's internal state
%   \State Send a {\sf Process-Saved-Batch} message to itself
% \EndProcedure
% \end{algorithmic}

% Instead of saving the remaining tuples in the internal state, alternatively it can send them as a data message to itself. However, when processing is done on a cluster and the data message may need to go over the network, a small control message is preferred.  

% Regardless of the implementation, the delay in processing control messages is reduced to:
% \begin{equation}
%     delay \approx n \tau  \beta.
% \end{equation}
% The reason is that only $\tau$ tuples from every batch of $\alpha$ tuples are processed before the control message.


% Table~\ref{table:control-msg-overhead} captures the overhead for different values of $\tau$ when a data set of 5 million tuples was sent through a workflow with each data batch of 1,000 tuples. $\tau = 1,000$ represents the default scenario when entire batch is processed as a whole without getting broken up. 

% \begin{table}[hbtp]
% \small{
% \begin{tabular}{|p{2.0cm}|p{2.5cm}|}
% \hline
% \textbf{$\tau$} & \textbf{Time taken (s)} \\
% \hline
% 1 & 31.6 \\ \hline
% 5 & 15.2 \\ \hline
% 10 & 11.1 \\ \hline
% 50 & 10.3 \\ \hline
% \textbf{1000} & \textbf{8.5} \\ \hline
% \end{tabular}
% }
% \textit{}
% \caption{Delay of processing a control message using solution 1.}
% \label{table:control-msg-overhead}
% \end{table}

%The worker saves handles \hl{CL: what "handles"?} to these threads and shares some state information with them.

\vspace{0.05in}
\noindent \textbf{Solution 2. Delegating data processing to a separate thread.} In the actor model, each actor is presumably single-threaded, and can do only one thing at a time. We extend this notion by allowing an actor to create its own thread (called {\em data-processing thread} or {\em DP thread} for short), with the purpose of concurrent computation. After receiving a data batch, a worker can create a DP thread (if not already existing) and offload the processing to it (Figure~\ref{fig:solution2-dpthread} (i) and (ii)). Once the processing is handed over to the DP thread, the worker is free to continue processing the next message in the mailbox. If the next message is also a data batch, and the DP thread is busy processing the previous batch, the new batch is stored in an internal queue (Figure~\ref{fig:solution2-dpthread} (iii)). If the next message is a control message such as {\sf Pause}, the worker can process it (Figure~\ref{fig:solution2-dpthread} (iv)) and tell this event to the DP thread by setting a shared variable {\sf Paused} to true.  The consequent actions of the DP thread will be described in Section~\ref{ssec:pause-and-resume}.  Similarly, when the worker sees a {\sf Resume} control message in the mailbox, it will set the variable to false to notify the DP thread.

\begin{figure*}[htbp]
	\vspace{-0.1in}
	\includegraphics[width=7in]{figs/solution2.pdf} 
	\caption{\label{fig:solution2-dpthread}
		Expedited processing of control messages using a DP thread.
	}
	\vspace{-0.1in}
\end{figure*}

% The pseudo code in Algorithm~\ref{alg:sol2-newthread} illustrates the details.

% \begin{algorithm}[ht]
%   \SetKwFunction{ProcessBatch}{Process-Batch}\SetKwFunction{ProcessControlSignal}{Process-ControlSignal}\SetKwFunction{ProcessBatchByThread}{Process-Batch-By-Thread}
  
%     \SetKwProg{myproc}{Procedure}{}{}
%     \myproc{\ProcessBatch{$batch$}}{
%         Create a DP thread if doesn't exist\;
%         Invoke \texttt{Process-Batch-By-Thread} and pass $batch$ to it\;
%     }{}
    
%     \myproc{\ProcessControlSignal{}}{
%     \uIf{$signal \equiv PAUSE $}{
%       $ pause \gets true $\;
%     }
%     \Else{
%       Process other signals\;
%     }
%     }{}
    
%     \myproc{\ProcessBatchByThread{}}{
%     \For{$i \gets 1$ \textbf{to} \texttt{batch.size()}} {
%         \uIf{$pause$}{
%             Save state and exit \;
%         }
%         \Else{
%             Process $batch[i]$\;
%         }
%     }
%     }{}
    
%   \caption{Solution 2}
%   \label{alg:sol2-newthread}
% \end{algorithm}

% Assuming that passing a data batch to a separate DP thread incurs an overhead of $\lambda$,  the delay of processing a control message enqueued behind $n$ data messages is:
% \begin{equation}
%     delay \approx n \lambda.
% \end{equation}

For these two solutions, the second one is preferred because its time involved in delegating a batch to a separate thread is much smaller than the time of processing $\tau$ tuples in the batch. Moreover, the approach achieves less delay without any increase in the number of messages. Therefore, we adopt solution 2 in the rest of the discussion.

% \hl{CL: we will remove this paragraph in the final version.} {\em Why not start another actor instead of thread?} A variation of solution 2 is starting another actor and offloading the processing to the new actor instead of a separate thread. However, this solution has an inbuilt problem. Say actor $A$ receives a data batch, creates actor $B$, offloads the processing to actor $B$, and exits. Now, when actor $A$ receives a control message, say {\sf Pause}, it has to tell actor $B$ to pause. However, the only way these two actors can communicate is using messages. If actor $A$ sends a control message to actor $B$, the control message will be put behind all the data messages in the mailbox of actor $B$. Thus, we are back at the problem we started with. The solution of ``creating threads'' does not have this problem because the actor communicates with the threads through shared states, and not messages.

{\bf DP thread checking {\sf Paused} variable.} The DP thread periodically checks the variable {\sf Paused} and pauses its data processing after seeing the value to be true. There are different granularities at which the DP thread can check this variable. The largest is batch granularity, where the check is done after processing every batch. A better option is to check the {\sf Paused} variable at the smaller granularity of tuples.  Notice that operators use an {\em iteration} model to process their received tuples and apply their computation logic on each tuple. Hence, the check for the {\em Pause} variable can be done before processing every tuple, which can reduce the response time for a pause request.

%The number of tuples ($\tau$) processed at one go, before a control check is done, is referred to as \emph{control-check granularity}. 
%Solution 2 implies that processing of data batches occurs on a different thread (DP thread) than the main worker actor thread. Therefore, the DP thread needs to pause processing of data when a {\sf Pause} message is processed by the main worker thread. 


% \begin{table}[bt]
% \small{
% \begin{tabular}{|p{2.0cm}|p{2.5cm}|p{2.5cm}|}
% \hline
% \textbf{$\tau$} & \textbf{Time taken} & \textbf{Time taken when $\tau=1000$} \\
% \hline
% 1 &  & \multirow{2}{*}{} \\ \cline{1-2}
% 5 &  & \\ \hline
% 10 &  & \\ \hline
% 50 &  & \\ \hline
% \end{tabular}
% }
% \textit{}
% \caption{Overhead incurred to implement control check granularity in actor model}
% \label{table:control-msg-overhead}
% \end{table}

\subsection{Saving and Loading Actor States}
\label{ssec:pause-and-resume}

% \vspace{0.05in}
% \noindent \textbf{Control check granularity.} 
% \hl{CL: Not sure whether I followed the details. Let's discuss F2F.} We fragmentize the execution of a data batch, in both the solutions mentioned above, to allow quick processing of control message. Specifically, in solution 1, we processed the data batch only $\tau$ tuples at a time. In the \texttt{Process-Batch-By-Thread} procedure of solution 2, we did a check for ``pause'' state change every tuple. However, this is also configurable and the check can be done every $\tau$ tuples. The number of tuples ($\tau$) processed at one go, before being interrupted, is referred to as \emph{control-check granularity}. 

% Assuming that smaller control check granularity results in faster processing of control messages and hence more real-time experience for users, is incorrect. For example, as discussed before, in solution 2, lesser $\tau$ leads to a higher number of messages in the entire engine, that can result in flooding of message channels. Thus, any subsequent control messages can take long time to process. However, the situation is different in case of solution 3. Here, the control-check granularity of 1 tuple in solution 3, is just a condition check and doesn't cause any extra messages to be produced. Therefore, the only limitation is an added overhead of condition check in each iteration. This overhead and slow execution is akin to execution of traditional C++/Java program in debug mode where it runs far slower than in non-debug mode.

When the DP thread observes that the {\sf Paused} variable is set to true, it needs to pause the processing of its data batch. One way to do the pause is to let this thread sleep and periodically wake up to check the variable to know if the thread should continue. This solution has two problems. 1) It wastes CPU cycles by periodically waking up and checking the variable. 2) Thread is occupied and cannot be used for other purposes. A better approach is that the DP thread saves all necessary states of data processing in the actor's internal state, then simply exits. When a {\sf Resume} message arrives, the main worker thread deploys a (possibly new) DP thread, which loads the saved states to resume the computation.  Next we consider various operators and study what state information should be saved for later resumption.

%Note that distributed implementation of operators to handle big data, especially relational operators, is a well studied problem and is not the focus of this section. This section solely focuses on answering the above two questions for various example operators and the discussion here can be generalized to other operators as well.

% We adopted Solution 4 to solve implement \emph{Control Check Granularity}. To implement relation operators using this method, the operators implementations will have to be granulated. After each \emph{Control Check Granule}, there can be a check for control message. These granulated implementations will be used by threads that actors offload the processing to. Next, we illustrate how different relational operators can be granulated. 

% An example UDF operator could implement advanced ML or NLP techniques.  

\vspace{0.05in}
\noindent \textbf{1. Non-blocking operators (e.g., selection, projection, and UDF operators)}:  In a non-blocking operator, each tuple is processed independently by the DP thread.  Thus the only information that needs to be saved is the index (or offset) of the next to-be-processed tuple in the batch. We call it the \emph{resumption-index}. When a {\sf Resume} message arrives, the main worker thread creates a new DP thread, which can locate the next tuple using the resumption-index.

\vspace{0.05in}
\noindent \textbf{2. Sort}: It is a blocking operator as it does not output results until it receives the entirety of the input data, as indicated by a special message called {\sf End-Of-Data}. One way to implement distributed sort in the actor model is to have two layers of workers. The first layer has multiple workers, each of which receives a subset of tuples and sorts them locally. The second layer contains a single worker that merges the sorted outputs of the first-layer workers.  We use this method to show how to save and load states, and the solution works for other distributed sort implementations as well.

A first-layer worker does its local sort using an algorithm such as {\sf InsertionSort}, {\sf MergeSort}, and {\sf QuickSort}. Take {\sf InsertionSort} as an example, which sorts tuples online as they arrive by maintaining a sorted list of received tuples.  When iterating over the tuples in a new input batch, it inserts each tuple into the sorted list. When pausing the execution, the DP thread saves the resumption-index, i.e., the offset of the next tuple in the batch to be processed next. If the first-layer worker uses an offline sorting algorithm such as {\sf MergeSort}, the worker needs to save all its received tuples till seeing an {\sf End-Of-Data} message, when the DP thread is invoked to do merge sort on the saved tuples. When pausing the execution, the DP thread saves the state of merge sort to resume the operation later.  The worker in the second layer merges the sorted outputs of first-layer workers to produce the final sorted results. It gets sorted input batches from all first-stage workers and iterates over them. When pausing the execution, the DP thread needs to store the resumption-index for each input batch.

\vspace{0.05in}
\noindent \textbf{3. Hash-based Join.} This operator consists of two phases, namely hash-building for one input table (say ``Table-A'') and probing the hash table using the tuples from the other table (say ``Table-B''). The input data is divided among the workers based on a global hash function, and each worker  receives tuples belonging to specific hash buckets from both tables. Each worker iterates over the received tuples of Table-A to build a local hash table. All Table-B tuples received by the worker before receiving the {\sf End-Of-Data} message for Table-A are saved in the worker's internal storage. When the worker receives an {\sf End-Of-Data} message for Table-A, it begins the second phase, in which it iterates over saved tuples as well as new tuples of Table-B to probe the hash table to produce results.

When a worker receives a {\sf Pause} message, its DP thread can be in one of the two phases. If it is in the hash-building phase, it saves its states related to building the hash table and the resumption index for the interrupted batch of Table-A. If the DP thread is in the probing phase, it saves the corresponding state and the resumption index from the interrupted batch of Table-B.

%In general, for any operator, if the worker implements the operator logic in two or more phases, then it needs to remember the phase it was in order to resume processing.

\vspace{0.05in}
\noindent \textbf{4. Ripple Join.}  To implement ripple join~\cite{conf/sigmod/HaasH99}, workers receive tuples belonging to specific hash buckets from both tables, and do the join in a single phase. In particular, a worker saves data batches of both tables. When it receives a data batch of one table, it joins the tuples of received batch with the saved tuples of the other table. This join method allows quicker forwarding of resulting tuples to the next operator compared to the hash-based join. 

Suppose the DP thread is joining a Table-A batch with the saved tuples of Table-B. When pausing its execution, the thread saves two resumption indices. The first index is of the tuple of the Table-A batch that was being processed, and the second index is of the tuple from the saved tuples of Table-B that was going to be checked next for join against the tuple of Table-A. When resuming, the worker passes the two indices to the new DP thread to resume the ripple join.

\textbf{5. GroupBy.} It can be implemented either using sorting or hashing.  As an example, consider a sort-based GroupBy implementation, which has two phases, namely phase 1 of sorting the table and phase 2 of grouping the tuples to form aggregates. Suppose we want to find the sum of an attribute \texttt{column-B} grouped by another attribute \texttt{Column-A}. In phase 1, the table is sorted by \texttt{Column-A}, and we can use the two-layer distributed sort approach described above to do the sorting. In phase 2, the sorted table is used to aggregate \texttt{column-B} for every distinct value of \texttt{Column-A}. This phase can be implemented by the second-layer worker in the distributed sort. 

%After it merges the sorted outputs of the first layer workers and produces an overall sorted order on \texttt{Column-A}, it can then iterate through this output and aggregate \texttt{column-B}. Therefore, Sort-based GroupBy can be implemented using two layers of workers, and the second layer worker does the dual task of merging the outputs of first layer and calculating the aggregates.

When pausing the execution, the DP thread of a first-layer worker saves the same information as in the sort implementation above.  The DP thread of the second-layer worker can be one of two stages, namely merging the sorted outputs or grouping. Similar to a worker of hash-based join, the second-layer DP thread first saves the stage it is in. If it is in the sorting stage, it also saves the information to resume the merging process.  If it is in the grouping phase, the thread needs to save the index of the tuple to be processed next from the sorted output, and the aggregates per group computed till now.

\vspace{0.05in}
\noindent {\em Remarks:} One general observation of these operators is that they are based on iterations to process income tuples, which provides an opportunity for the DP thread to check the {\sf Paused} variable and save related states in order for another thread to resume the computation as the place it was paused.

% \subsubsection{Checking for control message while batch is executing}
% In many cases, the user may need to do frequent pauses and wants the data message execution to interrupt if a control message is next in the queue. This is increasingly important if the time to process a batch is huge like in the later stages of Join where the new batch has to be joined with a huge table, or in the later stages of sort where a huge list has to be iterated to get the correct position of the incoming tuples. Therefore, we allow checking of control messages while a batch is executing. Since, checking of control messages during batch execution will cause a performance hit, we allow this only in debug mode. The experience is similar to running a program in debug mode, where the user sees runtime details, but the program execution is too slow.

% Our implementation uses signals to let batch execution know that a control message has arrived. In general, the actor, in order to process the batch of data messages, iterates through the batch and processes the tuples. At the start of each iteration, we check if there is a control message waiting. If yes, we save the state and stop the processing, to process the control message. After the control message is processed, we resume the processing of the interrupted data batch (unless the control message was a `pause` message). For the sake of simplicity, say the actor is sorting the incoming tuples using insertion sort.

% This is tricky to implement in actor model. The actor model specification, doesn't give an actor the ability to receive signals or leave a message in middle of processing and jump to some other message. So, we adopt a different way to achieve the above in our actor model based implementation of engine. The \emph{ProcessBatch} method of the \emph{SortActor} does receive the input batch, but it starts another thread (say Thread \emph{A}) to do the actual processing and exits the method. This is similar to a web server that starts a new thread to service the incoming request. Once, the \emph{ProcessBatch} method is exited, the \emph{SortActor} is free to process other received messages, while the processing of the batch takes place in thread \emph{A}. If a control message like \emph{Pause} comes before the batch has been processed, the \emph{SortActor} processes the \emph{Pause} message and turns the pause variable to \emph{true}. The pause variable is being observed by thread \emph{A}. As soon as the variable becomes \emph{true}, thread \emph{A} saves its state and exits.




==> chap4-maestro/sec1.tex <==
\chapter{Maestro: Result-aware Scheduling for Exploratory Data Analysis on Big Data}
\label{chap:maestro}

\section{Introduction}
\label{sec:maestro-introduction}


Big data processing systems have become quite popular in the last two decades. We have mentioned various examples of such systems in the previous chapters. We also discussed that these systems accept workflows broadly through two interfaces - programming APIs and GUIs. The input workflow is compiled and executed by the engine. 


The task to execute an input workflow to completion is performed by a scheduler. Scheduling a workflow involves decisions such as how to execute the various operators in the workflow and the resources to execute them on. A scheduler analyzes a workflow and comes up with an order to execute the operators. It also decides how many resources (such as CPU cores and memory) will be needed to execute these operators. Frameworks such as LSched~\cite{conf/sigmod/SabekUK22} and Decima~\cite{conf/sigcomm/MaoSVMA19} can help the scheduler decide the appropriate amount of resources to be assigned. Once the resource needs are determined, the scheduler may need to apply for a lease of the resources on shared clusters. Cluster managers such as YARN~\cite{conf/cloud/VavilapalliMDAKEGLSSSCORRB13} and Borg~\cite{conf/eurosys/VermaPKOTW15} have been developed to provide such leases.


The division of a workflow into multiple parts, each containing one or more operators, for scheduling depends on the type of execution. In batch-based execution adopted by systems such as Apache Hadoop~\cite{misc/hadoopmapreduce} and Apache Spark~\cite{misc/spark}, the workflow is broken down at data-shuffle boundaries~\cite{spark-stage} into a sequence of map and reduce phases. All the tasks of a phase should finish before the next phase starts. There are some optimizations to allow the reduce phase to partially overlap with the map phase using a slow-start configuration~\cite{misc/hadoop-mapreduce-configs}. On the other hand, in pipelined execution adopted by systems such as Apache Flink~\cite{misc/flink} and Hyracks~\cite{conf/icde/BorkarCGOV11}, the workflow is broken down at blocking links into a sequence of pipelined regions~\cite{misc/flink-pipelined-region-scheduling}. Blocking links are edges in a workflow DAG whose destination operator does not produce any output till it processes all the input data on that edge. Examples of blocking links are the build input of a two-phase {\sf HashJoin} operator and the input to {\sf GroupBy} operator. 



We discussed the benefits of pipelined execution in exploratory data analysis in Chapter~\ref{chap:reshape}. Pipelined execution allows the results to be produced quickly because an operator does not wait for its entire input data to be produced before processing the input and sending results to its downstream operators. For example, when a workflow containing a two-phase {\sf HashJoin} operator is executed in a pipelined mode, the {\sf HashJoin} operator starts executing and producing results as soon as the upstream operator producing probe input outputs initial results. \avinash{In contrast, when the workflow is executed in batch mode, the {\sf HashJoin} operator waits for the entire probe input to be produced before processing it. Note that in both the execution models, the {\sf HashJoin} operator does not produce any output while processing the build input.} In this chapter, we consider the pipelined execution setting to enable the users to see results quickly.


The problem of scheduling has been extensively studied in the literature, mainly from the perspective of increasing the end-to-end performance~\cite{conf/middleware/PengHHFC15, conf/debs/AnielloBQ13, conf/infocom/ChengCZGM17}. However, there is little research on the following important problem:

\begin{quote}
{\em In exploratory data analytics, how to consider the timing of results shown to the user when scheduling a workflow?}
\end{quote}


A few works are related to this problem. A work ranks the partitions of input data in the order of their likelihood to produce results and higher ranked partitions are processed first~\cite{conf/icde/EngOST03}. Other works focus on a particular operator such as join and customize the implementation of the operator so that it produces results quicker~\cite{conf/vldb/UrhanF01, conf/vldb/Lawrence05}. 

In this chapter, we take a different perspective. Considering a workflow DAG as an input in a pipelined execution setting, we explore how to divide the workflow into smaller parts that can be separately scheduled and how to schedule the different parts so that results are shown to the user quickly.


A simple way to divide a workflow into parts for scheduling is based on the blocking links as discussed above. However, such a simplistic division may lead to problems when operators such as union are present in the workflow (Section~\ref{sec:extending-to-union}). We propose a concept of dividing a workflow into several fine-grained regions that accommodate operators such as union. We also present an algorithm for creating a region graph that encapsulates the dependencies among the regions of a workflow.


There exist operators that expect the input data to arrive on their input links in a particular order and cause exceptions if that expectation is not met. For example, a two-phase {\sf HashJoin} operator requires the complete input to arrive on its build input link before input data arrives on its probe input link. To cater to such a join operator, the part of the workflow producing build input should execute completely before the part of the workflow producing probe input executes. However, in many cases, the build and probe input are produced by the same part of the workflow. Figure~\ref{fig:simple-self-join} shows such a workflow. Consider the execution of this workflow in the pipelined mode. When the {\sf Scan} operator starts producing data, both {\sf Filter1} and {\sf Filter2} process data and output the results to {\sf HashJoin} simultaneously, which causes an exception. Engines typically take a heuristic-based approach to handle such workflows. For example, Apache AsterixDB~\cite{asterix:website} adds materialization at an output of the operator that replicates the data, i.e., materialization is added on the link between the {\sf Scan} and the {\sf Filter2} operators. However, it can be seen in the figure that materialization can also be added to the link between the {\sf Filter2} and the {\sf HashJoin} operator. In this chapter, we identify the different places where materialization can be added in the workflow and examine their effect on the results shown to the user.

 \begin{figure}[htbp]
 \begin{center}
    % \vspace{-0.1in}
	\includegraphics[width=3.5in]{figures/maestro/simple-self-join.pdf}
% 	\vspace{-0.12in}
	\caption{\label{fig:simple-self-join}
		\textbf{A workflow where probe and build inputs may arrive at join simultaneously. This leads to an exception if the join operator expects build input to be processed completely before the probe input arrives.}
	}
% 	\vspace{-0.15in}
    % \vspace{-0.2in}
\end{center}
\end{figure}

In this chapter, we present a novel result-aware scheduling framework called \schfrmname that analyzes a workflow DAG to create regions in a result-aware manner that are executed in a pipelined execution setting. We make the following contributions. (1) Dividing the workflow into regions and creating a region graph: We present a technique to divide a workflow into fine regions that considers the existence of multi-pipelined input operators such as union in the workflow (Section~\ref{sec:schedule-a-workflow} and \ref{sec:extending-to-union}). We present an algorithm to create a region graph that encapsulates the dependencies among the regions of a workflow (Section~\ref{sec:schedule-a-workflow}). The region graph is used by the scheduler to decide the order of execution of the regions. (2) Enumeration of materialization choices: When there is a need for materialization, there may be multiple places in the workflow where the materialization can take place. We present an algorithm to enumerate all the options of materialization. (3) Result-aware materialization choice: We perform an analysis to compare the different choices of materialization from the perspective of result awareness.



\subsection{Related work}
\label{ssec:maestro-related-work}

\boldstart{Cluster resource managers.} When a cluster is shared by different applications, the applications need to interact with the resource managers to execute their tasks. Apache Hadoop YARN~\cite{conf/cloud/VavilapalliMDAKEGLSSSCORRB13} is a resource manager that publishes APIs that can be used by applications to send resource requests (e.g., CPU cores, memory) and receive resource leases to execute their tasks. Once the lease has been obtained the application takes care of placing the tasks to be executed on those resources. YARN allocates resources based on different policies such as FIFO, FAIR, and capacity-based scheduling. Mesos~\cite{conf/nsdi/HindmanKZGJKSS10} works in a fashion similar to YARN where it offers resources to application level schedulers. Borg~\cite{conf/eurosys/VermaPKOTW15} is a resource manager that accepts job requests and, unlike YARN and Mesos, also manages placing the tasks of a job on different machines. In contrast, \schfrmname focuses on the scheduling of a particular workflow and can contact the cluster resource managers to ask for the computational resources needed for execution.


\boldstart{Early result production.} Symmetric hash join~\cite{conf/pdis/WilschutA91,journals/debu/UrhanF00} aims towards early production of join results by keeping hash tables for both inputs in its state. When a tuple arrives from one input, it is used to probe the hash table of the other input. Early hash join~\cite{conf/vldb/Lawrence05} is a join algorithm that allows early production of results without much overhead on the total execution time. It runs in two phases where the first phase focuses on quickly producing results and the second phase focuses on reducing the execution time. Another way to produce data early is to rank the partitions of input data in the order of their likelihood to produce results and process the higher ranked partitions first~\cite{conf/icde/EngOST03}. In contrast, \schfrmname focuses on the execution of a workflow as a whole and is not specific to a particular operator. The techniques in \cite{conf/vldb/Lawrence05, conf/icde/EngOST03} can complement \schfrmname to get even better results.

\boldstart{Workflow schedulers.} The schedulers in Apache Hadoop and Apache Spark divide the workflow into a sequence of stages~\cite{spark-stage}. Each stage has a predefined parallelism that is equal to the number of tasks in that stage. Tasks are allocated to the computation nodes when the nodes become available~\cite{misc/spark-job-scheduling}. The scheduler in Apache Flink and Hyracks divides a workflow into a sequence of pipelined regions based on blocking links~\cite{misc/flink-pipelined-region-scheduling}. The pipelined regions, similar to stages, have predefined parallelism. In systems such as Apache Storm~\cite{apacheStorm}, the traffic of data during the execution of the workflow can be monitored to change the placement of operators and improve performance. R-Storm~\cite{conf/middleware/PengHHFC15} is a scheduler for Apache Storm that requires each task of a workflow to provide its resource needs and allocates them accordingly.  If a task receives data from another task in the workflow, then it tries to put them on the same node. A-scheduler~\cite{conf/infocom/ChengCZGM17} is a scheduler for Spark Streaming that follows a scheduling policy that does FIFO scheduling for dependent tasks in a workflow and FAIR scheduling for independent tasks. LSched~\cite{conf/sigmod/SabekUK22} and Decima~\cite{conf/sigcomm/MaoSVMA19} are query schedulers that use machine learning to predict how to schedule individual queries so as to reduce the overall execution time of the workload. Davos~\cite{journals/pvldb/ShangZBEKMRK21} uses a publish-subscribe pattern between operators for data transmission and schedules operators one at a time depending on which operator has pending input. It uses a priority-based scheduling strategy to execute the operator in a workflow that has its input ready and is nearest to the output. \schfrmname is different from the Davos scheduler because Davos assumes a publish-subscribe based execution, whereas \schfrmname assumes a pipelined-based execution. Most workflow schedulers focus on improving the performance of a workflow, i.e., reducing the total execution time. In contrast, \schfrmname approaches the scheduling problem from the perspective of result timing awareness.


==> chap4-maestro/sec2.tex <==
\section{Preliminaries}
\label{sec:maestro-preliminaries}

In this section, we introduce a running example and a few preliminary concepts that we refer to throughout this chapter.

\boldstart{Running Example.} Figure~\ref{fig:maestro-running-example}(a) shows a workflow, which will serve as our running example, where the user wants to analyze the effect of wildfires on people's perception of climate change. The user wants to analyze the text in the tweets from before, during, and after the wildfire season. The historical information about the count of past fires in various zipcodes is read by {\sf Scan1} operator. The zipcodes with no history of wildfires are filtered out. The resulting historical information is joined with the tweets on the zipcode attribute. The join is a two-phase {\sf HashJoin} operator, where the historical information is the build input and the tweet data is the probe input. The output of the join operator is input into an {\sf ML} operator that classifies the tweet text as being related to climate change or not. The result is plotted as stacked bar charts where the $x$ axis is the income range of zipcode and the $y$ axis is the proportion of tweets related and unrelated to climate change. For the tweets collected during the wildfire season, only those that have the word ``fire'' are input into the join operator. The tweets during the wildfire season are also plotted on a scatterplot operator to show their spatial distribution.

\begin{figure*}[htbp]
	\begin{center}
	    
	\includegraphics[width=6in]{figures/maestro/running-example.pdf} 
	\caption{\label{fig:maestro-running-example}
		\textbf{Analyzing climate change awareness in tweets before, during and after the wildfire season. The build inputs to join are shown in red. All joins are on the zipcode column. The ML operators determine if the tweet is about climate change.}
	}
		\end{center}

% 	\vspace{-0.2in}
\end{figure*}

As discussed in Chapter~\ref{chap:amber}, each operator physically corresponds to a set of workers that process input data and send output data to the workers of the downstream operators. There is a centralized controller that oversees the execution of the workflow. Next we define a few preliminary terms and concepts that will be used in this chapter.

\begin{definition}[Result operators]
We use the term {\em result operators} to refer to operators that produce tabular or visual results. These operators do not have any output links.
\end{definition}
In Figure~\ref{fig:maestro-running-example}, the {\sf bar chart} and the {\sf scatterplot} operators are result operators.

\begin{definition}[Blocking and pipelined links]
We call a link between two operators as {\em blocking} if the destination operator does not produce any output till it processes all the input data on that link. We call a link as {\em pipelined} if the destination operator starts producing output before it has processed all the input data on that link.
\end{definition}
For example, the build input link to a two-phase {\sf HashJoin} is a blocking link because the entire build input is needed to create a complete build hash table and no output is produced by the operator before that. The probe input link to a two-phase {\sf HashJoin} is a pipelined link because the operator may start producing output before it has processed the entire probe input. {\sf Sort} and {\sf GroupBy} operators are examples of operators that have just a single blocking input and no pipelined inputs.

\avinash{
\boldstart{Implementation of a {\sf HashJoin} operator.} In this chapter, we assume a specific implementation of the {\sf HashJoin} operator that we have in \amberfrmname, as explained next. 
}

==> chap4-maestro/sec3.tex <==
\section{Overview of \schfrmname scheduler}
\label{ssec:working-of-scheduler}

A workflow DAG input into the engine needs to be scheduled for execution by the scheduler. This section gives a high level overview of the working of the \schfrmname scheduler. The \schfrmname scheduler is a module inside the controller of the workflow as shown in Figure~\ref{fig:maestro-architecture}. 
% The scheduling policy is a pluggable module of the scheduler chosen prior to execution.
 
 \begin{figure}[htbp]
 \begin{center}
    % \vspace{-0.1in}
	\includegraphics[width=4in]{figures/maestro/architecture.pdf}
% 	\vspace{-0.12in}
	\caption{\label{fig:maestro-architecture}
		\textbf{Scheduling in \schfrmname}
	}
% 	\vspace{-0.15in}
    % \vspace{-0.2in}
\end{center}
\end{figure}
 
 The user submits a workflow to the data processing engine through an interface. The {\em region builder} compiles the workflow DAG to create a region graph. A region is a sub-DAG of the workflow and the region graph is a graph capturing the order in which the regions of a workflow should be executed. We discuss the concepts of region and region graph in detail in Section~\ref{sec:schedule-a-workflow}. The region graph is passed to the scheduler. The scheduler executes the regions according to the configured scheduling policy.

% The scheduler maintains a set of ready regions represented by $\omega$. In the running example, the initial set of ready regions is $\omega = \{r_1\}$. 

The scheduler receives certain {\em events} from the user or the workers executing the operators. Upon the receipt of an event, the scheduler makes scheduling decisions based on the policy. For example, when the user sends a command to start the workflow, the scheduler receives an event to begin the execution of the workflow. During the execution of a workflow, the scheduler receives various events about the execution status of the regions. An example of an event received during execution is the completion of a worker of an operator. The scheduler uses these events to decide on the scheduling of other regions.

% In the running example, it executes $r_1$, which is the only ready region at the beginning. When a region starts executing, it is taken out of $\omega$ and put into a set of running regions. The completion of a blocking link sends another event to the scheduler. For example, the completion of the blocking link between {\sf Filter1} and {\sf HashJoin1} sends an event to the scheduler. The completion of this link makes $r_2$ ready because it is the only blocking link between $r_1$ and $r_2$. After receiving this event, the scheduler makes the next scheduling decision according to its policy. For example, the scheduler can start the execution of $r_2$ when it becomes ready. A different policy can be to wait for the completion of $r_1$ and then start the execution of $r_2$.

==> chap4-maestro/sec4.tex <==
\section{Building a region graph in \schfrmname}
\label{sec:schedule-a-workflow}

In this section, we describe how an input workflow is scheduled in \schfrmname. First, we define the concepts of a region and dependencies between regions (Section~\ref{ssec:defining-regions-and-dependencies}). Then, we describe the process to create a region graph, which captures the dependencies between regions, from a workflow DAG (Section~\ref{ssec:creating-region-graph}) and also discuss how to schedule a region graph. There are two assumptions in this section which we remove in later sections. The first assumption is that the workflow does not contain any operators that have more than one pipelined input link. An example of such an operator is the union operator. The second assumption is that the region graph does not have any cycles. We remove the first and the second assumptions in Sections~\ref{sec:extending-to-union} and \ref{sec:cycles-in-region-graph}, respectively.

\subsection{Regions and their dependencies}
\label{ssec:defining-regions-and-dependencies}

\schfrmname divides a workflow DAG into sub-DAGs called ``regions,'' each of which can be separately scheduled. We define the concepts of region, dependencies between regions, and other related terms below.

\begin{definition}[Region]
A {\em region} is a maximal weakly connected sub-DAG of the workflow DAG $W$ in which all the operators are connected with only pipelined links. All the operators in a region process input and produce output data simultaneously. 
\end{definition}
The running example consists of $4$ pipelined regions marked by dotted oval shapes in Figure~\ref{fig:maestro-running-example-with-regions}(a). All the operators in a region are scheduled together by \schfrmname. \avinash{Note that from the perspective of implementation, the {\sf HashJoin1}, {\sf HashJoin2}, and {\sf HashJoin3} operators are active when region $r_1$ is executing so that they can receive and process the output of {\sf Filter1}. However, in this chapter, we do not consider them to be a part of $r_1$ for the purpose of simplicity of explanation. This way of representing regions is also adopted by systems such as Flink where operators do not belong to the region of their upstream operators producing blocking input~\cite{misc/flink-pipelined-region-scheduling}.}

% All the operators and links except the blocking links belong to one of the regions. The blocking links may be used to build dependencies between different regions in a workflow as we will discuss soon.

\begin{figure*}[htbp]
	\begin{center}
	    
	\includegraphics[width=6in]{figures/maestro/running-example-with-regions.pdf} 
	\caption{\label{fig:maestro-running-example-with-regions}
		\textbf{Regions and region graph from the running example workflow. Blocking input links are in red.}
	}
		\end{center}

% 	\vspace{-0.2in}
\end{figure*}

\begin{definition}[Execution of a region]
The {\em execution} of a region refers to the deployment of the operators of the region on the cluster and the subsequent processing of input data by the operators.
\end{definition}
If a region has not been executed yet, it is called an {\em unscheduled region}.

\begin{definition}[Sources of a region]
The {\em sources} of a region are the operators in the region that have no pipelined input links. In other words, the operator should have either no input links at all or only blocking input links. 
\end{definition}
The operators with no inputs are the scan operators. Examples of operators with only blocking inputs are {\sf GroupBy} and {\sf Sort}. When an operator has only blocking inputs, it receives input data from an operator in a different region. When a region is executed, the sources of the region produce the data to be processed by the region. In the running example, {\sf Scan1}, {\sf Scan2}, {\sf Scan3}, and {\sf Scan4} are the sources of $r_1$, $r_2$, $r_3$, and $r_4$, respectively. For instance, {\sf Scan1} has no input links and produces the data processed by the operators of $r_1$.

\begin{definition}[Completion of a link and region]
A link between operators is said to be {\em completed} if all the data on the link has been received by the destination operator. A region is said to be {\em completed} if all its operators have processed all their input data and produced all their output data.
\end{definition}

\begin{definition}[Dependency between regions]
A region $Y$ is said to be {\em dependent} on another region $X$ if there exists at least one blocking link $l$ from an operator in $X$ to an operator in $Y$ and all the data on $l$ should be completely received before the operators in $Y$ start executing. 
\end{definition}
In Figure~\ref{fig:maestro-running-example-with-regions}(a), regions $r_2$, $r_3$, and $r_4$ all depend on $r_1$ because $r_1$ produces the build input for the {\sf HashJoin} operators in the regions $r_2$, $r_3$, and $r_4$.

\begin{definition}[Ready region]
Let a region $r$ depend on a set of regions represented by $D$. The region $r$ is said to be {\em ready} when all the regions in $D$ have completed and all blocking links to $r$ from the regions in $D$ have also completed.  When a region is ready, it can be executed.
\end{definition}


% \boldstart{Region DAG.} The region DAG ($\mathcal{R}$) for a workflow is a DAG with the regions of the workflow as its vertices and the dependencies between the regions as its edges. An edge from a region $X$ to a region $Y$ in the region DAG means that $Y$ is dependent on $X$. Figure~\ref{fig:maestro-running-example-with-regions}(b) shows the region DAG for the running example.

\subsection{Creating a region graph}
\label{ssec:creating-region-graph}


We mentioned in Section~\ref{ssec:defining-regions-and-dependencies} that the various regions of a workflow may have dependencies among them. When a region has to be scheduled, all the regions that it depends on should have already  completed. Thus, the scheduler has to follow an order when executing the regions of a workflow. This order is captured in the region graph for a workflow, which we define below.

\begin{definition}[Region graph]
The {\em region graph} for a workflow is a graph with the regions of the workflow as its vertices and the dependencies between the regions as its edges. An edge from a region $X$ to a region $Y$ in the region graph means that $Y$ is dependent on $X$.
\end{definition}

Algorithm~\ref{alg:region-graph-creation} describes the process to create a region graph from a workflow DAG $W$. The algorithm first creates the regions of the workflow. These regions form the vertices of the region graph. Then, the algorithm adds edges to the region graph. These edges represent the dependencies between the regions. Specifically, the algorithm starts by removing the blocking edges from $W$ to get the graph $W^{'}$ (line~\ref{algline:remove-blocking}). In the running example workflow, this means removing the three red colored edges between {\sf Filter1} and the three {\sf HashJoin} operators. Each weakly connected component of $W^{'}$ forms a region. These regions are put into a set $V$ (line~\ref{algline:find-components}), which forms the vertices of the region graph $G$ (lines~\ref{algline:vertices-of-graph-s}-\ref{algline:vertices-of-graph-f}). The four regions for the running example workflow are shown in Figure~\ref{fig:maestro-running-example-with-regions}(a). Lines~\ref{algline:topological-order} - \ref{algline:added-edges} encapsulate the process to add edges to the region graph. Let $O$ be a topologically ordered sequence of operators in $W$ (line~\ref{algline:topological-order}). The operators in $O$ are sequentially considered and the following is done for each of them. Let the region to which an operator $o$ belongs be $r_o$ (line~\ref{algline:region-of-o}). We find the blocking input links to the operator $o$. Let $b$ be a blocking input link to $o$ and $r_b$ be the region to which the source operator of $b$  belongs (lines~\ref{algline:blocking-input-o}, \ref{algline:blocking-input-o-region}). An edge is added from $r_b$ to $r_o$ in $G$ (line~\ref{algline:add-edge-to-g}). This is repeated for each blocking input link of $o$. In the running example, the three {\sf HashJoin} operators are the only ones with blocking inputs. The operators {\sf HashJoin1}, {\sf HashJoin2}, and {\sf HashJoin3} belong to the regions $r_2$, $r_3$, and $r_4$ respectively. The source operator of the blocking inputs to them ({\sf Filter1}) belongs to the region $r_1$. Therefore, edges are added from $r_1$ to $r_2$, $r_3$, and $r_4$. The final region graph is shown in Figure~\ref{fig:maestro-running-example-with-regions}(b).

\begin{algorithm}[htbp]
\caption{\hl{Region graph creation.} \label{alg:region-graph-creation}}
        \KwIn{$W \gets$ Workflow DAG}
        \KwOut{G: Region graph}
        
     $W^{'} \gets$ Remove blocking edges from $W$ \\ \label{algline:remove-blocking}
     $V \gets$ Maximal weakly connected components of $W^{'}$ \tcp{Each component is a region.}  \label{algline:find-components}
     Initialize $G$ to an empty graph \\
     \ForEach{component c in V}{ \label{algline:vertices-of-graph-s}
        Add a vertex in $G$ corresponding to the region representing $c$
     } \label{algline:vertices-of-graph-f}
     $O \gets$ A topological order of operators in $W$ \\ \label{algline:topological-order}
     \ForEach{operator o in O} {
        $r_o \gets$ region of operator o \\ \label{algline:region-of-o}
        \ForEach{blocking input link b to o}{ \label{algline:blocking-input-o}
            $r_b \gets$ region of source operator of link b \\ \label{algline:blocking-input-o-region}
            Add an edge from the vertex of region $r_b$ to $r_o$ in $G$, if not already there \label{algline:add-edge-to-g}
        }
     } \label{algline:added-edges}
     return $G$
\end{algorithm}

We assume that there is no requirement on the order in which the inputs from blocking links should be processed by an operator. The only requirement is that all the inputs on blocking links should be processed by an operator before the operator starts receiving input from its pipelined input links. If there exist any other order requirements among the inputs, Algorithm~\ref{alg:region-graph-creation} can be easily extended to capture those requirements. Note that Algorithm~\ref{alg:region-graph-creation} also works for operators that only have one input link which is blocking. Examples of such operators are {\sf GroupBy} and {\sf Sort}. For such an operator (say $o$), the algorithm adds an edge from the region containing the upstream operator of $o$ to the region containing $o$.

\boldstart{Scheduling a region graph.} The regions must be scheduled in a topological order based on the region graph, in order to ensure that a region is executed only when all the regions it depends on have been executed. In order to obtain a topological order, the region graph should not have any cycles, i.e., it should be a DAG. As mentioned before, we assume in this subsection that there is no cycle in the region graph. This assumption will be removed in the later sections. In the running example, the region graph obtained does not have any cycles and can be scheduled. An example of the order of execution of the regions in the running example is $r_1$, $r_2$, and $r_3$.


==> chap4-maestro/sec5.tex <==
\section{Extending to operators with multiple pipelined inputs}
\label{sec:extending-to-union}

In Section~\ref{sec:schedule-a-workflow}, we described the process of scheduling workflows in \schfrmname using regions and the region graph. We assumed in that section that the workflow does not contain any operators that have more than one pipelined input link such as {\sf union}. We remove that assumption in this section. First, we take an example workflow containing an operator with multiple pipelined inputs and show a problem in scheduling the regions of the workflow (Section~\ref{ssec:finer-regions-need-union}). Then, we refine the concept of region to solve the problem (Section~\ref{ssec:refine-region-concept}). We discuss the way to find the regions of a workflow according to the refined concept. There is no change in the way of finding the dependencies among the regions.


\subsection{Need for finer-granularity regions}
\label{ssec:finer-regions-need-union} 

Figure~\ref{fig:finer-regions-need} shows a workflow to create a scatterplot of the selling price ({\em sp}) and the cost price ({\em cp}) of items belonging to different categories and compare the profit margins for the items. The probe input ({\sf Scan2}) containing the selling prices of items is joined with the build input ({\sf Scan1}) containing the cost price of the items on the {\em item} attribute and the output is projected to have the {\em item}, {\em category}, and {\em sp} attributes. The output from {\sf Scan1} and {\sf Project} are merged in the {\sf Merge} operator, which adds an extra column specifying if the tuple is from {\sf Scan1} or {\sf Project}. The merged data is visualized on a scatter plot.

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=6in]{figures/maestro/finer-regions-need.pdf} 
	\caption{\label{fig:finer-regions-need}
		\textbf{Workflow with a {\sf Merge} operator with multiple pipelined inputs. When the workflow contains a single region and the region is started, both the scan operators start producing data simultaneously, which causes the {\sf HashJoin} operator to raise an exception.}
	}
		\end{center}
% 	\vspace{-0.2in}
\end{figure*}


The \schfrmname scheduler executes the workflow by executing its regions. In order to find the regions of the workflow in Figure~\ref{fig:finer-regions-need}, we remove the blocking input link to {\sf HashJoin} and find the maximal weakly connected components of the DAG. The entire DAG remains weakly connected after removing the blocking edge. Hence, there is only one region in this workflow. If \schfrmname tries to schedule this region, it sends {\em start} messages to the sources of the region, namely {\sf Scan1} and {\sf Scan2}. Both receive a {\em start} message and begin to produce data. This causes an exception in the {\sf HashJoin} operator because the operator expects the probe input to arrive only after the build input has been completely processed. 


A way to schedule the workflow without causing any exception is to first send a {\em start} message to the {\sf Scan1} operator. The data from {\sf Scan1} goes into {\sf HashJoin} as the build input and also to the {\sf Merge} operator that processes it and passes the output to the {\sf Viz} operator. After {\sf Scan1} has produced data completely and the data has been processed by the {\sf HashJoin} operator, a {\em start} message is sent to the {\sf Scan2} operator that provides the probe input to {\sf HashJoin}. The output of {\sf HashJoin} then goes to the {\sf Viz} operator through the {\sf Project} and {\sf Merge} operators. Thus, the exception can be avoided if instead of executing the workflow as a single region, we execute the two regions with {\sf Scan1} as the source of the first region and {\sf Scan2} as the source of the second region. Based on this intuition, we refine the concept of regions in the next subsection to allow \schfrmname to correctly schedule workflows containing operators with multiple pipelined inputs.

\subsection{Improving the region concept}
\label{ssec:refine-region-concept}

The concept of regions in Section~\ref{sec:schedule-a-workflow} is coarse and allows for multiple sources to exist in a region. If multiple sources exist in a region, the scheduler starts all of them at the same time, which leads to exceptions when the sources produce blocking and pipelined inputs of an operator, as shown in Figure~\ref{fig:finer-regions-need}. In order to have control over the scheduling order of each source, we refine the concept of region and make its granularity finer by allowing only one source per region. On a high level, this refinement results in the coarse regions from Section~\ref{sec:schedule-a-workflow} being divided into multiple smaller regions. 

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=6in]{figures/maestro/finer-regions-example.pdf} 
	\caption{\label{fig:finer-regions-example}
		\textbf{Regions in a workflow with a {\sf Merge} operator containing multiple pipelined inputs. Each region contains only one source. Thus, Scan1 and Scan2 belong to different regions and can be separately scheduled.}
	}
		\end{center}
% 	\vspace{-0.2in}
\end{figure*}

\begin{definition}[Region]
A region is a sub-DAG of the workflow that starts at a source operator and contains all the operators reachable from the source operator using only pipelined edges.
\end{definition}

It should be noted that when a workflow does not contain any operator with multiple pipelined inputs, the old definition of region in Section~\ref{sec:schedule-a-workflow} also allows only one source operator per region. Thus, the new definition of region is just a generalization of the old definition to ensure single source per region when the workflow contains operators with multiple pipelined inputs.

For the workflow in Figure~\ref{fig:finer-regions-need}, the refinement results in two regions $r_1$ and $r_2$ as shown in Figure~\ref{fig:finer-regions-example}. The {\sf Merge} and {\sf Viz} operators belong to both regions. These new regions become the vertices of the region graph. Lines~\ref{algline:topological-order} - \ref{algline:added-edges} of Algorithm~\ref{alg:region-graph-creation} can be followed to find the dependencies between the regions and create a region graph. In the example in Figure~\ref{fig:finer-regions-example}, the {\sf HashJoin} operator introduces an edge from region $r_1$ to $r_2$. The scheduler executes the workflow according to the region graph, by executing $r_1$ and then $r_2$. The scheduler sends a {\em start} message to {\sf Scan1} to start executing $r_1$. When $r_1$ has completed, the scheduler sends a {\em start} message to {\sf Scan2}. This way of executing the workflow avoids the exception in {\sf HashJoin} that was mentioned in Section~\ref{ssec:finer-regions-need-union}. 


\boldstart{Updated algorithm to create regions and region graph.} Lines~\ref{algline:remove-blocking} and \ref{algline:find-components} of Algorithm~\ref{alg:region-graph-creation} need to be updated to find regions according to the refined concept that accommodates operators with multiple pipelined input. First, we find all the operators in the workflow DAG that have no pipelined inputs. Each of these operators is the source of their own regions. These regions are the vertices of the region graph. Once the regions have been identified, lines~\ref{algline:topological-order} - \ref{algline:added-edges} of Algorithm~\ref{alg:region-graph-creation} can be followed to find the dependencies between the regions and create a region graph. Note that an operator can now belong to multiple regions, as shown in Figure~\ref{fig:finer-regions-example}. Thus, lines~\ref{algline:region-of-o} and \ref{algline:blocking-input-o-region} may yield a set of regions for the operator $o$ and the source operator of link $b$. We add edges from each region containing $o$ to each region containing the source operator of link $b$ in line~\ref{algline:add-edge-to-g}.


==> chap4-maestro/sec6.tex <==
\section{Dealing with cycles in the region graph}
\label{sec:cycles-in-region-graph}

In Section~\ref{sec:schedule-a-workflow}, we assumed that there is no cycle in the region graph. In this section, we remove that assumption. We first show an example workflow whose region graph contains a cycle (Section~\ref{ssec:cycle-cause}). When such a cycle exists, a topological order for the regions does not exist, which makes scheduling the regions infeasible. Therefore, the workflow DAG needs to be modified in a way that the resulting region graph does not have any cycles. We discuss the different ways to modify the workflow (Section~\ref{ssec:modify-workflow-approaches}). One of the ways to modify the workflow is to introduce materialization operators. We enumerate the different options where the materialization operators  can be placed in the workflow (Section~\ref{sssec:materialization-choices}) and discuss how it affects result awareness (Section~\ref{ssec:mat-choice-result-aware}).

\subsection{Cause of cyclic region graph}
\label{ssec:cycle-cause}

Figure~\ref{fig:cyclic-region-simple-workflow} shows a workflow DAG and its corresponding region graph. The workflow tries to find a new department for the employees in the machine learning department and their managers. It visualizes the count of employees and managers by the new departments they have been allotted to. There is only one region in the workflow whose source is the {\sf Scan} operator. The {\sf HashJoin} expects to first completely receive and process its build input from {\sf Filter1}. Then, it expects to receive the probe input from {\sf Filter2}. Since both {\sf Filter1} and {\sf Filter2} belong to the same region $r_1$, the region graph has a cycle, as shown in the figure. Such a cyclic region graph cannot be scheduled.

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=4.8in]{figures/maestro/cyclic-region-simple-workflow.pdf} 
	\caption{\label{fig:cyclic-region-simple-workflow}
		\textbf{Workflow with cyclic region graph. When there is a cycle in the region graph, there is no feasible schedule of regions.}
	}
		\end{center}
% 	\vspace{-0.2in}
\end{figure*}

The key problem in the workflow in Figure~\ref{fig:cyclic-region-simple-workflow} is that when a {\em start} message is sent to the source of $r_1$ ({\sf Scan}), the input flows from both {\sf Filter1} and {\sf Filter2} into the {\sf HashJoin} operator simultaneously, which causes an exception. Next, we see how to modify the workflow to solve this problem.

\subsection{Modification of workflow and region graph}
\label{ssec:modify-workflow-approaches}

In order to enforce the requirement of the probe input of {\sf HashJoin} arriving after the build input, the two inputs need to be produced by different regions. The region producing the build input will need to be scheduled first, followed by the region producing the probe input. We discuss two ways to modify the workflow and create new regions, namely replication and materialization, in Section~\ref{sssec:possible-ways-to-modify-workflow}. We describe the process to enumerate different materialization choices in Section~\ref{sssec:materialization-choices}.

\subsubsection{Possible ways of creating new regions}
\label{sssec:possible-ways-to-modify-workflow}

There are different ways to modify the workflow so that the probe input for {\sf HashJoin} arrives from a different region than the build input. One way is to remove the {\sf Duplicate} operator and replicate the operators {\sf Scan1} and {\sf ML1} to supply the data to {\sf Filter2} as shown in Figure~\ref{fig:cyclic-region-simple-workflow-solving}(a). This creates two regions $r_1$ and $r_2$, and $r_2$ has a dependency on $r_1$. This way incurs the overhead of repeated computation. For example, in Figure~\ref{fig:cyclic-region-simple-workflow-solving}(a), the input data is processed by the same ML operator twice. 

Another way to create a new region is to introduce materialization. Materialization is introduced on a link by adding a materialization writer and a materialization reader operator to the link. The materialization writer writes all the data produced by the source operator of the link to a memory or disk. The materialization reader reads the data from the storage and outputs it to the destination operator of the link. In Figure~\ref{fig:cyclic-region-simple-workflow-solving}(b), materialization writer and reader operators have been put between the operators {\sf Filter2} and {\sf HashJoin}. The introduction of materialization also creates two regions $r_1$ and $r_2$, where $r_2$ is dependent on $r_1$. The {\sf Scan} operator is the source of $r_1$ and the materialization reader operator ({\sf MR}) is the source of $r_2$. The region graph for the two ways discussed above is the same and is shown in Figure~\ref{fig:cyclic-region-simple-workflow-solving}(c). We focus on the case where computational resources are more expensive than storage. We will follow the materialization way to modify the workflow DAG in case of cyclic region graphs.

% The materialization operators can also be put at other places and we will discuss about that soon.

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=\linewidth]{figures/maestro/cyclic-region-simple-workflow-solving.pdf} 
	\caption{\label{fig:cyclic-region-simple-workflow-solving}
		\textbf{Modifying workflow in Figure~\ref{fig:cyclic-region-simple-workflow} to create an acyclic region graph.}
	}
		\end{center}
% 	\vspace{-0.2in}
\end{figure*}

\subsubsection{Enumerating the materialization choices}
\label{sssec:materialization-choices}

In Figure~\ref{fig:cyclic-region-simple-workflow-solving}(b), the materialization operators were placed between the {\sf Filter2} and the {\sf HashJoin} operators. However, another choice is to place them between the {\sf ML1} and {\sf Filter2} operators. Both choices create two regions and result in the same region graph as shown in Figure~\ref{fig:cyclic-region-simple-workflow-solving}(c). In general, there can be multiple choices where materialization operators can be placed in a workflow. We are going to describe the process to enumerate all those choices.

For simplicity, we consider the case where the region graph has a single cycle. We first give an intuitive explanation of how to enumerate the different materialization choices by giving an example. Then, we give a formal approach for enumerating the choices.

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=\linewidth]{figures/maestro/cyclic-region-mat-choices.pdf} 
	\caption{\label{fig:cyclic-region-mat-choices}
		\textbf{Enumerating all the materialization choices. {\sf J1}, {\sf J2}, {\sf J3}, and {\sf J4} are {\sf HashJoin} operators. {\sf D1} and {\sf D2} are replication operators. {\sf M1} and {\sf M2} are ML operators. {\sf S} is scan, {\sf F} is filter, and {\sf U} is a union operator.}
	}
	\end{center}
\end{figure*}

\boldstart{Intuition.} Figure~\ref{fig:cyclic-region-mat-choices}(a) shows the outline of a workflow with its regions marked. The corresponding region graph containing a cycle is shown in Figure~\ref{fig:cyclic-region-mat-choices}(b). The problem exists at the operator {\sf J4} that receives its probe input from the region $r_2$ before the build input arrives from the region $r_4$. In order to solve this problem, we use materialization to modify the workflow DAG in such a way that the probe input to {\sf J4} can be delayed. The materialization should split the region $r_2$ into two parts, thereby ``cutting off'' the flow of data from $r_2$ into the probe input of {\sf J4}.  This is similar to the network flow problem where one needs to determine the cut edges in the graph that make a target vertex unreachable from the source vertices~\cite{fulkerson1962flows}. In our case, the target vertex is the operator whose probe input has to be cut off ({\sf J4}) and the cut edges are the links where data has to be materialized. Figure~\ref{fig:cyclic-region-mat-choices}(c) shows materialization added to the link between {\sf U} and {\sf J4}. It cuts off the probe input to {\sf J4} and divides the region $r_2$ into two parts $r_2^{1}$ and $r_2^{2}$ as shown in Figure~\ref{fig:cyclic-region-mat-choices}(d).

A key consideration while adding the materialization is that the materialization should cut off the probe input to {\sf J4} from $r_2$, but the build input to {\sf J2} (in $r_3$) should still come from $r_2$. If this does not happen and the build input to {\sf J2} is produced by the newly created region, then there still will be a cycle in the region graph. Thus, we need to identify the sub-DAG of the workflow where the materialization can happen such that it cuts off the probe input to {\sf J4} from $r_2$ but does not impact the build input to {\sf J2} from $r_2$. This sub-DAG for the workflow in Figure~\ref{fig:cyclic-region-mat-choices}(a) is shown in Figure~\ref{fig:cyclic-region-mat-choices}(e). The figure also shows $6$ different sets of cuts, each of which disconnects {\sf D1} and {\sf J4}. These cuts form the $6$ materialization choices. Each cut includes a set of edges where the data has to be materialized. The choices $1$ and $6$ consist of one edge only, which means that they require a single materialization writer and reader operators. When one of these two options is chosen, the region $r_2$ is broken into $r_2^{1}$ and $r_2^{2}$. The single materialization reader becomes the source of the region $r_2^{2}$ and the resulting region graph is shown in Figure~\ref{fig:cyclic-region-mat-choices}(f). The choices $2$, $3$, $4$, and $5$ consist of two edges each, which means that they require two materialization writer and reader operators, one pair on each edge. When one of these four options is chosen, the region $r_2$ is broken into three regions $r_2^{1}$, $r_2^{2}$ and $r_2^{3}$. The two materialization readers become the source of the regions $r_2^{2}$ and $r_2^{3}$, and the resulting region graph is shown in Figure~\ref{fig:cyclic-region-mat-choices}(f).


\boldstart{Formal approach.} Consider that $W$ is a workflow DAG and $C$ is its region graph containing a cycle as output by Algorithm~\ref{alg:region-graph-creation}. Algorithm~\ref{alg:adding-mat-cylic-region-graph} adds materialization to $W$ to obtain a modified workflow DAG $W_m$ whose region graph does not have a cycle. Let $O$ be a topological order of operators in $W$ (line~\ref{algline:formal-topological}). We sequentially iterate through the operators in $O$ and check if the operator belongs to a region in the cyclic part of $C$. Let the region in the cyclic part of $C$ whose operator is first found in $C$ be $r_a$ (lines~\ref{algline:formal-find-ra-start}-\ref{algline:formal-find-ra-end}). Figure~\ref{fig:cyclic-region-mat-choices-formal-approach-outline}(a)
shows an example outline of the workflow $W$ with region $r_a$ marked. Let $r_x$ and $r_b$ be the regions before and after $r_a$ in the cycle in $C$, respectively (lines~\ref{algline:formal-find-rx} and \ref{algline:formal-find-rb}). Let $J_a$ be the operator in $r_a$ responsible for the edge from $r_x$ to $r_a$ being added by the Algorithm~\ref{alg:region-graph-creation} in the region graph (line~\ref{algline:formal-find-ja}). Let $J_b$ be the operator in $r_b$ receiving the blocking input from $r_a$ (line~\ref{algline:formal-find-jb}). As explained above, the materialization should cut off the input to $J_a$ from $r_a$ but not impact the blocking input to $r_b$ from $r_a$.

\begin{algorithm}[htbp]
\caption{\hl{Adding materialization to a workflow with a cyclic region graph.} \label{alg:adding-mat-cylic-region-graph}}
        \KwIn{$W \gets$ Workflow DAG}
        \KwIn{$C \gets$ Region graph of $W$ with a cycle}
        \KwOut{$W_m$: Modified workflow DAG after adding materialization to $W$}
    
    $O \gets$ A topological order of operators in $W$ \\ \label{algline:formal-topological}
    \ForEach{operator o in O}{ \label{algline:formal-find-ra-start}
        \If{o belongs to a region $r$ in the cyclic part of $C$} {
            $r_a \gets$ r \\
            break \\
        }
    } \label{algline:formal-find-ra-end}
    $r_x \gets$ Region that is before $r_a$ in the cycle in $C$ \\ \label{algline:formal-find-rx}
    $r_b \gets$ Region that is after $r_a$ in the cycle in $C$ \\ \label{algline:formal-find-rb}
    $J_a \gets$ Operator in $r_a$ responsible for the edge $r_x \rightarrow r_a$ in $C$ \\ \label{algline:formal-find-ja}
    $J_b \gets$  Operator in $r_b$ receiving the blocking input from $r_a$ \\ \label{algline:formal-find-jb}
    $S_a \gets$ Source of $r_a$ \\ \label{algline:formal-find-sa}
    $G_a \gets$ Sub-DAG of W containing operators and edges on all paths from $S_a$ to $J_a$ using pipelined edges \\ \label{algline:formal-find-ga}
    $G_b \gets$ Sub-DAG of W containing operators and edges on all paths from $S_a$ to $J_b$ via the blocking input of $J_b$ \\ \label{algline:formal-find-gb}
    $G_f \gets G_a - G_b$ \\ \label{algline:formal-find-gf}
    $P \gets $ Operators that are the source of the edges in $G_f$ with no source vertex \\ \label{algline:formal-find-p}
    $G^{'}_f \gets G_f + P$ \\ \label{algline:formal-find-gf'}
    $E \gets$ A cut-edge set in $G^{'}_f$ that makes $J_a$ unreachable from all operators in $P$ \\ \label{algline:formal-find-e}
    $W_m \gets$ Modify $W$ by adding materialization operators to all the edges in $E$ \\ \label{algline:formal-find-wm}
\end{algorithm}


\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=6in]{figures/maestro/cyclic-region-mat-choices-formal-approach-outline.pdf} 
	\caption{\label{fig:cyclic-region-mat-choices-formal-approach-outline}
		\textbf{Understanding the formal approach to find the sub-DAG where materialization is to be added. A sub-DAG of operators has been shown in the region $r_a$ as an example to understand the algorithm.}
	}
	\end{center}
\end{figure*}


Let $S_a$ be the source of the region $r_a$ (line~\ref{algline:formal-find-sa}). We find all the paths from $S_a$ to $J_a$ using only pipelined edges. Let the sub-DAG containing all the operators and edges on these paths be $G_a$ ((line~\ref{algline:formal-find-ga})) (Figure~\ref{fig:cyclic-region-mat-choices-formal-approach-outline}(a)). Let the sub-DAG containing all the operators and edges on all paths from $S_a$ to $J_b$, via the blocking input of $J_b$, be called $G_b$ (line~\ref{algline:formal-find-gb}) (Figure~\ref{fig:cyclic-region-mat-choices-formal-approach-outline}(a)). Let $G_f = G_a - G_b$ (line~\ref{algline:formal-find-gf}) (Figure~\ref{fig:cyclic-region-mat-choices-formal-approach-outline}(b)). On a high level, the graph $G_f$ is the part of $r_a$ that produces pipelined input for $J_a$, but does not produce the blocking input for $J_b$. The sub-DAG $G_f$ will have one or more edges that do not have an operator at their source, as shown in the figure. These edges emerge from operators in $G_b$. Let the set of operators in $G_b$ that these edges emerge from be called $P$ (line~\ref{algline:formal-find-p}). We add operators in $P$ to the sub-DAG $G_f$ to create $G_f^{'}$ (line~\ref{algline:formal-find-gf'}), as shown in Figure~\ref{fig:cyclic-region-mat-choices-formal-approach-outline}(c). Once the sub-DAG $G_f^{'}$ has been identified, we need to identify all possible cut-edges sets~\cite{fulkerson1962flows} that make the operator $J_a$ unreachable from the operators in $P$ (line~\ref{algline:formal-find-e}). Each element of the set is a materialization choice and contains a collection of edges where materialization can be added. We choose one materialization option and apply it to $W$ to get $W_m$ (line~\ref{algline:formal-find-wm}).

% \begin{figure*}[htbp]
% 	\begin{center}
% 	\includegraphics[width=4in]{figures/maestro/cyclic-region-mat-choices-formal-approach.pdf} 
% 	\caption{\label{fig:cyclic-region-mat-choices-formal-approach}
% 		\textbf{Illustrating the formal approach to find materialization choices in the workflow in Figure~\ref{fig:cyclic-region-mat-choices}(a)}
% 	}
% 	\end{center}
% \end{figure*}

\subsection{Result-aware materialization choice selection}
\label{ssec:mat-choice-result-aware}

We saw how to enumerate different materialization choices in Section~\ref{ssec:modify-workflow-approaches}. In this section, we discuss how to consider result awareness while choosing a materialization option. We assume that there is a single cycle in the region graph and there is a single result operator in the workflow. We first define first response time, which is used as a metric for result awareness in this chapter. Then, we discuss how to choose a materialization option that gives a good first response time.

\subsection{First response time}
\label{ssec:first-response-time}

In exploratory analysis, the users want to quickly observe some initial output from the result operators. This allows the users to find issues in the analysis early without waiting for the entire workflow to finish executing~\cite{journals/pvldb/ShangZBEKMRK21}. Consider the following scenario. In the running example, when $r_3$ runs, the user may observe that the scatterplot operator contains many tweets related to other types of fires different from wildfire. Since the goal of the analysis is to determine whether wildfires lead to climate change awareness, the user may decide to add more keywords to the {\sf Filter2} operator to make the tweets more relevant to wildfire.

Considering a workflow with a single result operator, we define the {\em first response time} as follows. It is the time required from the start of execution of a workflow to the time when the result operator has produced a specific number of tuples (say, $d$). We denote the first response time by $\tau(d)$, where $d$ is the number of tuples that the result operators should produce. For simplicity, we consider $d=1$ in this chapter.

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=4in]{figures/maestro/first-response-time-def.pdf} 
	\caption{\label{fig:first-response-time-def}
		\textbf{The outline of a workflow showing regions. The sink operator in the last region. For first response time, we consider the time to completely execute all regions except the region containing the sink. For the region containing the sink, the time to produce only a single tuple is considered in the calculation of the first response time.}
	}
	\end{center}
\end{figure*}

\boldstart{First response time for a sequence of regions.} Let $r_a \rightarrow r_b \rightarrow r_c \rightarrow \cdots \rightarrow r_x $ be a sequence of regions (e.g., a topological order of regions from an acyclic region graph), where the result operator is present in $r_x$ (Figure~\ref{fig:first-response-time-def}). Assume each region in the sequence is completed before the next region begins execution. Let $t(r_i)$ represent the time to execute a region $r_i$ completely and $t(r_i(1))$ represent the time to produce a single tuple from the result operator in $r_i$. Then, the first response time for the sequence of regions is,
$$
\tau(1) = t(r_a) + t(r_b) + t(r_c) + \cdots + t(r_x(1)).
$$

\subsection{Choosing a materialization option}
\label{ssec:materialization-option-choice}

We now use the above description of first response time to discuss how to choose a materialization option. The goal is to choose an option that would reduce the first response time. 

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=4in]{figures/maestro/first-response-time-def-example.pdf} 
	\caption{\label{fig:first-response-time-def-example}
		\textbf{The outline of modified workflows showing regions when materialization is added to the workflow in Figure~\ref{fig:cyclic-region-mat-choices}(a). When there are more than one regions containing the sink, the first response time includes the minimum time among those regions to produce a single tuple.}
	}
	\end{center}
\end{figure*}

\boldstart{Explanation using example.} Let us consider the example region graph with a cycle shown in Figure~\ref{fig:cyclic-region-mat-choices}. When materialization options $1$ or $6$ are chosen, two new regions $r_2^{1}$ and $r_2^{2}$ are created out of $r_2$, and $r_2^{2}$ has the result operator (Figure~\ref{fig:first-response-time-def-example}(a)). In this case, the first response time is:
$$
\tau(1) = t(r_1) + t(r_2^{1}) + t(r_3) + t(r_4) + t(r_2^{2}(1)). 
$$
Note that the structure of $r_2^{1}$ and $r_2^{2}$ depend on which option is chosen. Thus, $t(r_2^{1})$ and $t(r_2^{2}(1))$ depend on which option is chosen. The time for the execution of other regions is not affected by the materialization choice. When materialization options $2$, $3$, $4$ or $5$ are chosen, three new regions $r_2^{1}$, $r_2^{2}$ and $r_2^{3}$ are created out of $r_2$, and both 
$r_2^{2}$ and $r_2^{3}$ have the result operators (Figure~\ref{fig:first-response-time-def-example}(b)). In this case, the first response time is:
$$
\tau(1) = t(r_1) + t(r_2^{1}) + t(r_3) + t(r_4) + min (t(r_2^{2}(1)), t(r_2^{3}(1))).
$$
Note again that the materialization option affects the structure of $r_2^{1}$, $r_2^{2}$ and $r_2^{3}$ and consequently the times $t(r_2^{1})$, $t(r_2^{2}(1))$ and $t(r_2^{3}(1))$. The execution times of other regions are unaffected. 

Query time estimation can be done to estimate $\tau(1)$ resulting from a materialization option. For a region $r$, $t(r)$ can be predicted by estimating the total query execution time~\cite{conf/icac/GuptaMD08,conf/icde/WuCZTHN13} for the query represented by the operator DAG in $r$. Similarly, $t(r)(1)$ can be predicted by estimating the time to get the first few results~\cite{conf/cikm/BayardoM96}. We choose the materialization option among the $6$ choices that has the least predicted $\tau(1)$.

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=4in]{figures/maestro/first-response-time-def-general.pdf} 
	\caption{\label{fig:first-response-time-def-general}
		\textbf{Example to help understand the generalization of first response time when a materialization choice $c$ is chosen in a region $r$. The region $r_c^1$ has to be fully executed, and any of the regions $r_c^2$, $r_c^3$, $\cdots$ has to produce a single tuple to get the first tuple out of the sink.}
	}
	\end{center}
\end{figure*}

\boldstart{Generalization.} In general, a materialization choice $c$ breaks a region $r$ into two sets of regions: 1) a single region $r_c^1$ that has the source of $r$ as its source and 2) a set of regions $\{r_c^2, r_c^3, \cdots\}$  that have the materialization readers as their sources. Let $\tau_c(1)$ be the first response time when the option $c$ is chosen. There are two cases to be considered when defining $\tau_c(1)$, depending on whether the result operator was in region $r$ before materialization or not. If the result operator was in region $r$, then the result operator will be part of all the regions in $\{r_c^2, r_c^3, \cdots \}$. Thus, these regions need to execute only partially for the first tuple to be produced from the result operator. On the other hand, if the result operator was not in $r$, then it will not be in any of the newly created regions. Thus, all the newly created regions will have to execute completely before the region with the result operator starts executing. Thus, we define $\tau_c(1)$ as the following:
$$ 
\tau_c(1) = \begin{cases} 
      T + t(r_c^1) + min(t(r_c^2(1)), t(r_c^3(1)), \cdots), & \text{ result operator} \in r \\
      T + t(r_c^1) + t(r_c^2) + t(r_c^3) + \cdots,  & \text{ result operator} \notin r, 
      \end{cases}
$$
where $T$ is a constant that denotes the time spent on regions other than $r$, which are not affected by materialization. The chosen materialization option is the one that has the smallest estimated $\tau_c(1)$.


==> chap4-maestro/sec7.tex <==
\section{Experiments}
\label{sec:maestro-exp}

We performed experiments to show the presence of cyclic region graphs and the presence of operators containing multiple pipelined inputs in workflows. We also performed experiments to showcase the effect of materialization choice on the first response time.

\subsection{Presence of cyclic region graphs and operators with multiple pipelined inputs}
\label{ssec:exp-analyze-workflows}

We analyzed $21$ workflows to detect the presence of cyclic region graphs and operators containing multiple pipelined inputs. For the workflows with cyclic region graphs, we also evaluated the number of cycles in their region graphs, the number of materialization choices for each cycle and whether there were any overlapping materialization choices among the cycles. We did the analysis on publicly available workflows from $3$ commercial workflow-based data processing systems - Alteryx, RapidMiner, and Dataiku - and the workflows in our Texera system. Sample workflows from the systems are shown in Figures~\ref{fig:alteryx-exp-image}, \ref{fig:rapidminer-exp-image}, \ref{fig:dataiku-exp-image}, and \ref{fig:texera-exp-image}. The results of the analysis are shown in Table~\ref{table:exp-analyze-workflows}.

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=4.8in]{figures/maestro/alteryx-image.png} 
	\caption{\label{fig:alteryx-exp-image}
		\textbf{An Alteryx workflow with cyclic region graph.}
	}
		\end{center}
% 	\vspace{-0.2in}
\end{figure*}

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=4.8in]{figures/maestro/rapidminer-image.png} 
	\caption{\label{fig:rapidminer-exp-image}
		\textbf{A RapidMiner workflow with cyclic region graph.}
	}
		\end{center}
% 	\vspace{-0.2in}
\end{figure*}

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=5.7in]{figures/maestro/dataiku-image.jpeg} 
	\caption{\label{fig:dataiku-exp-image}
		\textbf{A Dataiku workflow with cyclic region graph.}
	}
		\end{center}
% 	\vspace{-0.2in}
\end{figure*}

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=5in]{figures/maestro/texera-image-1.png} 
	\caption{\label{fig:texera-exp-image}
		\textbf{A Texera workflow with cyclic region graph.}
	}
		\end{center}
% 	\vspace{-0.2in}
\end{figure*}


\begin{table}[htbp]
% \vspace{-0.09in}
\centering
\small{
\begin{tabular}{|C{1.9cm}|C{2cm}|C{1.3cm}|C{3cm}|C{2.5cm}|C{3cm}|}
% \begin{tabular}{|l|l|l|l|}
\hline
{\bf System} & {\bf \# Operators} & {\bf \# Cycles} & \textbf{\# Mat choices} & \textbf{\# overlapping choices} & \textbf{\# Multi-pipelined input operators} \\ \hline
\multirow{7}{*}{Alteryx} & 26 & 2 & 6 in each cycle & 1 & 0 \\ \cline{2-6}
& 102 & 1 & 1 & 0 & 13 \\ \cline{2-6}
& 19 & 1 & 1 & 0 & 2 \\ \cline{2-6}
& 34 & 1 & 1 & 0 & 2 \\ \cline{2-6}
& 9 & 1 & 3 & 0 & 0 \\ \cline{2-6}
& 14 & 1 & 4 & 0 & 0 \\ \cline{2-6}
& 10 & 1 & 3 & 0 & 0 \\ \hline \hline
\multirow{6}{*}{RapidMiner} & 10 & 2 & 2 in first cycle, 1 in second cycle & 0 & 0 \\ \cline{2-6}
& 10 & 1 & 2 & 0 & 0 \\ \cline{2-6}
& 9 & 2 & 2 in first cycle, 1 in second cycle & 0 & 0 \\ \cline{2-6}
& 13 & 1 & 2 & 0 & 0 \\ \cline{2-6}
& 5 & 0 & 0 & 0 & 1 \\ \cline{2-6}
& 19 & 2 & 2 in each cycle & 0 & 1 \\ \hline \hline
\multirow{3}{*}{Dataiku} & 31 & 1 & 4 & 0 & 0 \\ \cline{2-6}
& 45 & 0 & 0 & 0 & 1 \\ \cline{2-6}
& 32 & 1 & 1 & 0 & 0 \\ \hline \hline
\multirow{5}{*}{Texera} & 30 & 1 & 3 & 0 & 0 \\ \cline{2-6}
& 8 & 1 & 1 & 0 & 0 \\ \cline{2-6}
& 8 & 1 & 1 & 0 & 0 \\ \cline{2-6}
& 9 & 0 & 0 & 0 & 1 \\ \cline{2-6}
& 10 & 0 & 0 & 0 & 1 \\ \hline
\end{tabular}
}
\textit{}
\caption{Analyzing the workflows from various workflow processing systems.}
% \vspace{-0.2in}
\label{table:exp-analyze-workflows}
\end{table}

The analysis shows that there are many publicly available workflows that have cyclic region graphs and contain operators with multiple pipelined inputs. The existence of such workflows in multiple data processing systems motivates the need for the concepts of finer-granularity regions and materialization choices discussed in Section~\ref{sec:extending-to-union} and \ref{sec:cycles-in-region-graph}.

\subsection{Effect of materialization choice on first response time}
\label{ssec:exp-mat-choice-first-response-time}

We took two workflows of similar structure and showed the effect of materialization choice on the first response time of the workflows. 

\boldstart{Data and workflows.} We used two workflows as shown in the Figure~\ref{fig:thesis-exp-workflows}. The workflows used two different sets of tweets as input datasets. Workflow $W1$ used a dataset of $372$ tweets and workflow $W2$ used a dataset of $3.1K$ tweets. The datasets used were small because both the workflows contained expensive machine-learning based operators that took considerable time to process each tweet. Workflow $W1$ processes the tweets using two machine-learning based operators that add labels to the tweets specifying whether the text of a tweet is related to climate change and whether the text suggests action to be taken regarding climate change. The outputs of the two operators are then joined on the {\em id} column to create a single tuple containing both labels for a tweet. Workflow $W2$ finds the tweets related to the opioid tramadol. These tweets are then joined with their reply-tweets using the {\em in-reply-to-id} attribute. Each tuple output of the {\sf HashJoin} operator contains a tweet about tramadol and one of its reply tweets. The sentiment label of the reply-tweet is also present that has been added by the {\sf Sentiment Analysis} operator. The output of {\sf HashJoin} is plotted on a spatial graph with edges between a tweet and its reply. The reply-tweet location is colored according to its sentiment. 

\begin{figure*}[htbp]
	\begin{center}
	\includegraphics[width=4in]{figures/maestro/thesis-exp-workflows.pdf} 
	\caption{\label{fig:thesis-exp-workflows}
		\textbf{Workflows used in the experiment to analyze the effect of materialization choices on the first response time. The blue triangles represent the materialization choices in the workflows.}
	}
	\end{center}
\end{figure*}

\boldstart{Experimental Setting.} The experiments were carried out on GCP on a single {\em n2-highcpu-32} machine containing $32$ CPU cores, $32$ GB RAM and $100$ GB HDD disk running Ubuntu 18.04.5 LTS. All the operators were given $2$ workers except the machine-learning based UDF operators in $W1$ which were given $4$ workers because they were expensive.

\boldstart{Materialization choices of W1}. The workflow $W1$ had two materialization choices shown in the Figure~\ref{fig:thesis-exp-workflows}. The first-response time when choice $1$ was used was $247$ seconds. The first-response time when choice $2$ was used was $710$ seconds. This shows that the choice $1$ is better. The reason is that when choice $2$ was used, the two expensive machine-learning based operators belonged to the same region and executed simultaneously. This led to competition between them for resources and slowed down computation.

\boldstart{Materialization choices of W2}. The workflow $W2$ also had two materialization choices. The selectivity of the {\sf Regex} operator was low because only a few tweets contained tramadol. The first-response time when choice $1$ was used was $361$ seconds. The first-response time when choice $2$ was used was $307$ seconds. The reason for the difference in first-response time is explained next. When choice $1$ was used, the {\sf Regex} operator belonged to a region that started execution after the sentiment analysis processed the entire data. Since the {\sf Regex} operator had low selectivity, it produced the first output after a considerable time. When choice $2$ was used, {\sf Regex} and {\sf Sentiment Analysis} operators belonged to the same region and data was processed by the {\sf Regex} operator alongside {\sf Sentiment Analysis} without adding much overhead. When the next region began execution, the first tuple was immediately output from {\sf HashJoin}.

Thus, we got lower first-response time when using choice $1$ for $W1$ and choice $2$ for $W2$. This experiment shows that the materialization choices do play a role in the first-response time.



==> chap4-maestro/sec8.tex <==
\section{Conclusion}
\label{sec:maestro-conclusion}

In this chapter, we presented a scheduling framework called \schfrmname. We showed how it divides a workflow into regions that can be separately scheduled. We described an algorithm to create a region graph that encapsulates the region dependencies. We showed the need for finer regions when the workflow contains multiple pipelined input operators. We showed that the the region graph can only be scheduled when it is acyclic and discussed examples where the region graph has cycles. We discussed how to use materialization to create an acyclic region graph from a cyclic region graph. We showed how to enumerate various choices for materialization. We introduced first response time as a metric of result awareness and discussed how the materialization choices differ from the perspective of result awareness. We presented experiments that motivated the concepts of fine-granular regions and materialization choices and showcased the effect of materialization choice on the first-response time.

